Cheater's Bowl: Human vs. Computer Search Strategies for Open-Domain Question Answering

For humans and computers, the first step in answering an open-domain question is retrieving a set of relevant documents from a large corpus. However, the strategies that computers use fundamentally differ from those of humans. To better understand these differences, we design a gamified interface for data collection -- Cheater's Bowl -- where a human answers complex questions with access to both traditional and modern search tools. We collect a dataset of human search sessions, analyze human search strategies, and compare them to state-of-the-art multi-hop QA models. Humans query logically, apply dynamic search chains, and use world knowledge to boost searching. We demonstrate how human queries can improve the accuracy of existing systems and propose improving the future design of QA models.

==> scripts/style-check/common-typos <==
a the                % phrase double article
 pt                  % syntax ? I guess avoid straggling pt's that escape tex?
[ ],                 % syntax whitespace before comma seems wrong.
Figure Figure        % phrase pizza pizza.
[ ]-[ ]              % syntax a hyphen surrounded by space should probably be an emdash '---'
[0-9]-[0-9]          % syntax use an endash '--' for ranges
[0-9]ms              % syntax put a space between the number and the unit.
[^egs]\. [a-z]       % syntax a period usually ends a sentence, and sentences should start with a capital; doesn't apply for i.e.,
\.  [a-z]            % syntax a period usually ends a sentence, and sentences should start with a capital; "i.e." should have a comma following.
[a-z]\.\.            % syntax double period is rarely right, use \ldots for ellipsis
[^\\]"               % syntax use fancy quotes
\beg\.               % syntax should be e.g. as in "examples given"
from to\b            % phrase haven't used this properly.
help help            % phrase double word, that probably means the author paniced
of of                % phrase apparent double word.
the affect           % phrase should probably be 'the effect'
the the              % phrase apparent double word.
there too few        % phrase there are too few?
was not was          % phrase pretty much a joke if this gets matched.
we we                % phrase it would be oi oi in french, I guess.
with on              % phrase probably wrong.
with with            % phrase apparent double word.
[\n ]--[\n ]         % syntax that's an en-dash, you want an em-dash: "---"
my my                % phrase unlikely that's what you want, at least without a comma. (doesn't work across newlines)
>From                % syntax be careful when you email .tex files.  I've seen this slip through into submissions.
e\.t\.c\.            % syntax it's et cetera; use etc.
such as like         % phrase pick one
<<<<<<< .            % syntax CVS conflict!
=======              % syntax CVS conflict!
>>>>>>> [0-9]        % syntax CVS conflict!
e\.g\.[\n ]          % syntax should be followed with a comma, as e.g. can be read as "for example" (thanks JZ!)
i\.e\.[\n ]          % syntax should be followed with a comma, as i.e. can be read as "that is" (thanks JZ!)
[ ]\.[\n ]           % syntax stray period?
further more         % phrase one word: furthermore
safe guard           % phrase one word: safeguard
that be              % phrase mistake.
can not              % phrase cannot
only only            % phrase double word
is is                % phrase double word.
they shows           % phrase argh, mistake.
less that than       % phrase typo damage
from from            % phrase double word score
in in                % phrase "in" (common mistake)
not not              % phrase argh.
it it                % phrase argh.
to illicit           % phrase "to elicit" -- illicit is always an adjective.
c\.f\.               % phrase actually, it's cf., and you'd like cf.\ (backslash space)
this lead to         % phrase "led to" if past tense, "leads to" if present.
on on                % phrase double word.
has is               % phrase choose
description their    % phrase saw this, clearly wrong.
including:  % syntax I prefer no colon after including, which already says a list is coming.
[a-z]\([A-Z]  % syntax put a space before parens, even when introducing acronyms.
without and without % phrase saw this.
can be result       % phrase saw this typo.



==> scripts/style-check/foolish-phrases <==
(quite|more|very|most) unique    % phrase unique is.
(quite|more|very|most) abstract  % phrase abstract is.
tangible view                    % phrase mix that metaphor some more.
for e\.g\.                       % phrase e.g. includes "for".
begs the question                % phrase unless you're very clever: "raises the question": http://alt-usage-english.org/excerpts/fxbegthe.html
high rate of speed               % phrase local news-speak.
especially necessary             % phrase 'especially important', necessary may be an absolute like unique.
how will it effect % phrase you likely meant "affect"
how it will effect % phrase you likely meant "affect"
insure proper performance % phrase "ensure"
especially true                  % phrase 'especially important', true may be an absolute like unique.
to affect change                 % phrase "effect" change;  I read this on a poster.
higher results                   % phrase maybe higher performance or higher values.
is more general then the         % phrase probably "than"
upper bounding                   % phrase "limiting" or "setting an upper bound on"
in principal                     % phrase likely, "in principle"
literally like                   % phrase literally means no simile.  
design principal  % phrase likely, "design principle" 
different from 	    	   	 % phrase unlike

==> scripts/style-check/latex-checking <==
\{\\em [^\}]*[^\}\/]\}[:]    % syntax use \emph{} or explicit italic correction {\em foo\/}
\{\\em [^\}]*[:\.,]\}        % syntax punctuation at the edges of italic text is not italicized
[A-Z]{2,10}\.[ ]*[\n ][ ]*[A-Z]  % syntax intersentence spacing should be used if a sentence ends with an acronym: "FOO\\@."
\\etal[^{]                   % syntax it's good practice to use \etal{} to avoid bad spacing
\\caption\[[^\]]*[^\.]\]     % syntax short caption should end with a period.
\\caption\[.*CCDF.*\]        % syntax short caption should not include graph type.
\\caption\[.*CDF.*\]         % syntax short caption should not include graph type.
\\caption\[.{0,25}\]         % syntax short caption should not be too short.
th century                   % syntax use textsuperscript
[ ]---[ ]                    % syntax the em-dash should be right up against the words.
[ \n]---[ \n]                % syntax the em-dash should be right up against the words.
^---[ \n]                    % syntax the em-dash should be right up against the words.
[ \n]---$                    % syntax the em-dash should be right up against the words.
[ \n]--[ \n]                 % syntax the en-dash should be between numbers.
^--[ \n]                     % syntax the en-dash should be between numbers.
[ \n]--$                     % syntax the en-dash should be rbetween numbers.
,[~ ]\\etal                  % syntax no comma before etal (unless Smith, Martinez, \etal)
\\etal\{\}'s                 % syntax eew.
\\(sub)?section\{[A-Z][^}]*[ ][a-z]{5,40}[^}]*\} % syntax subsection headers should be initial capped.
\\(sub)?section\{[A-Z][^}]*[^:][ ]{1,}(With|A|An|Is|And|For|To|The)[ ][^}]*\} % syntax some words needn't be capitalized
[ ]\\footnote                % syntax no space before footnote.
\\footnote\{.*\}.            % syntax footnotes after punctuation
,,                           % syntax double comma is unlikely to be intentional.
cf\.[^\\]                    % phrase cf. should get an escaped space "\ "
et al\.[^\\]                    % phrase et al. should get an escaped space "\ "
[<>]  % syntax a less than or greater than outside math mode shows other characters.
in (section|table|figure) \\ref % phrase should have ~ before ref
section~\\ref % capitalize capitalize section when saying Section 6.
table~\\ref % capitalize capitalize section when saying Table 6.
figure~\\ref % capitalize capitalize section when saying Figure 6.
\\(sub)?section\{Intro\} % syntax spell it out.
,''                          % syntax punctuation outside quotes
\.\.\.                       % syntax use \dots

==> scripts/style-check/my-rules <==
#  such may be abused to blacklist certain words even spelled correctly.
# capitalize is case sensitive, and also bracketed by non-word.
# phrase and spelling are case insensitive, but bracketed by non-word characters.
# syntax is case sensitive but not bracketed by non-word; probably best if used with regexes.
\bet al\.[^}]        % syntax use the \etal{} command instead. (or write one to italicize)
\bet\. al\.          % syntax use the \etal{} command, "et" needs no dot (et alii). (or write one to italicize)
\bc\.f\.\b             % syntax should be cf. for "confer" (latin for compare)
\b$i\)[^$]              % syntax leave the paren in math mode -- should be $i)$
\b$ii\)[^$]             % syntax leave the paren in math mode -- should be $ii)$
\b$iii\)[^$]            % syntax leave the paren in math mode -- should be $iii)$
\b$iv\)[^$]             % syntax leave the paren in math mode -- should be $iv)$
\b$v\)[^$]              % syntax leave the paren in math mode -- should be $v)$
\ban [b-df-gj-np-tv-z] % syntax probably meant to use "a" instead of "an", though there are exceptions.
\ban [B-DF-GJ-NP-TV-Z][^A-Z/] % syntax probably meant to use "a" instead of "an", though there are exceptions (like acronyms).
\b[Aa] [aeiouAEIOU](?!se|ni|A|ur|RL|ti|ne|DP) % syntax probably meant to use "an" instead of "a", though there are exceptions. (user, useful, AA, unified, uniform, unique, Europe, one, UDP; n/a doesn't work, so use {n/a})
This allows           % phrase tie more explicitly: This (x) allows...
we find               % phrase omit "we find"
we found              % phrase omit "we found"
try and               % phrase "try to", though if you're using try as a noun in a compound sentence, this rule is wrong.
impact of             % phrase not a useful metaphor; try evaluation, success, effect, value.
including [^\.]*etc\. % syntax "including" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
includes [^\.]*etc\.  % syntax "includes" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
and etc\.             % phrase come on. learn some latin.
AT&T                  % syntax you poor thing, this won't compile.
doesn't               % phrase be formal.
be occur              % phrase what happens when I'm indecisive about what follows "can"
up until              % phrase "until"
one or more           % phrase probably redundant -- nonzero is probably implied.
is comprise(d|s) of   % phrase you probably mean "is composed of" because "comprises" is more a synonym for "contains" 
will be significantly different % phrase "will differ significantly" for active voice
More importantly,     % phrase probably means the order is wrong: put important stuff first.
todo                  % ignoredcommand
texttt                  % ignoredcommand
jbgcomment              % ignoredcommand
lkfcomment              % ignoredcommand
due to space constraints % phrase don't whine.
this paper % phrase can be ambiguous if talking about someone else's paper whether you mean the one youre writing or the one you're talking about..
the above             % phrase horrible phrase that must be expunged.  you might use "these" instead, but best to make the sentence stand alone.
referred to above     % phrase "these".
(all|the|of) [0-9][ ] %  phrase use words for numbers in phrases.
clearly shows         % phrase "clearly" is usually much.
grows larger          % phrase is "grows smaller" possible?  grows.
guarantee as much as possible % phrase then not really a guarantee "provide"
affects negatively   % phrase "hurts" or "harms"
rely upon % phrase rely on is good enough
relies upon % phrase relies on is good enough
record route packets? % phrase hyphenate record-route packets
record-route; % phrase leave record route alone if not modifying something else
we accomplish this  % phrase verbose way to get active voice.
refers to the % phrase you're being wimpy in the definition.  use "is"
\\emph\{[a-zA-Z ]*\} refers to % syntax you're being wimpy in the definition.
loss off % phrase loss of?
this could % phrase this "what" could
with that has % phrase probably just one
simply % phrase probably isn't.
to get to % phrase "to reach"?
latency benefit % phrase reduction
latency improvement % phrase reduction
shed insight % phrase 'shed light' would seem the metaphor.
increasingly more % phrase redundant
I\.e\. % syntax starting a sentence with i.e. is just ugly.
E\.g\. % syntax starting a sentence with e.g. is just ugly.
in the large % phrase if large is a noun, bad.  if it's an adjective, fine.
encapsulates with % phrase seen it, don't know what it means.
when working with % phrase just say "with"
it is true that	  % phrase usually can delete
LDA % phrase convention put in small caps
(F|f)indings (show|indicate|suggest)	% phrase delete or make more specific

==> scripts/style-check/networking-research <==
IPs                  % phrase should be IP addresses
[Rr]ate-limits       % spelling "rate limits" has no hyphen, only "rate-limited"
best effort          % phrase hyphenate best-effort service.
deliver route        % phrase jargon redundancy
euclidean % capitalize Euclidean.
interdomain          % spelling inter-domain
internet             % capitalize unless talking about an internet other than the Internet
intradomain          % spelling intra-domain
log-normal           % spelling lognormal is one word.
pareto               % capitalize
ttl                  % capitalize
weibull              % capitalize proper name.
PoP                  % syntax I think POP looks less annoying.
PoPs                 % syntax I think POP looks less annoying.
http[ ]              % capitalize capitalize HTTP.
linux                % capitalize capitalize Linux
Internet[^\.]*Internet % syntax avoid Internet twice in the same sentence?
zipf                 % capitalize capitalize the guy's name.


==> scripts/style-check/passive-voice <==
it is possible to                   % phrase passive voice, try: "can"
are identified by                   % phrase passive
is shown                            % phrase passive.
is not included in                  % phrase maybe this is passive
there (are|is) [^\.:;]* (that|in)   % phrase maybe this is passive
can be evaluated                    % phrase avoid passive: I evaluated
can be observed                     % phrase avoid passive: are visible
# is needed                         % phrase passive voice
is used to                          % phrase go active voice, or subsititute "helps"
(are|were) needed[^\?]              % phrase passive voice
(is|are) presented in               % phrase "appears in", or reword to avoid passive voice
it is possible that                 % phrase "may"
(is|are) (depicted|illustrated|sketched) in  % phrase thats passive voice
(is|are) shown in                   % phrase "shows"
as can be seen in                   % phrase X shows that Y.
there needs to be                   % phrase passive voice in a bad way.
was designed                        % phrase passive voce.
it may be                           % phrase passive "it"
it is important that                % phrase passive; replace with X is important because Y.


==> scripts/style-check/verbose-phrases <==
a large number of                   % phrase you mean "many"
a substantial number of             % phrase how substantial?  most?  or just enough that can't be ignored?
an insufficient number of           % phrase "too few"
a significant number of             % phrase one is significant.   consider "prohibitive" if the number is sufficient to be problematic.
a number of                         % phrase getting the verb agreement for this useless phrase is tricky.
a number of different               % phrase use "different" (should have a high score)
a small number of                   % phrase you mean "few"
a low number of                   % phrase you mean "few"
a relatively low number of                   % phrase you mean "few"
actually                            % spelling probably doesn't add
to an extent                        % phrase you can probably remove
and instead                         % phrase replace with but?
be done                             % phrase if "X of Y can be done", try "Y can be Xed"; it's already passive voice.
combining multiple                  % phrase as opposed to "combining one?"
aggregating multiple                % phrase "aggregating"
do this                             % phrase probably verbose if you use a pronoun for what you're doing
exists[ ]                           % phrase probably no better than "is", but end of sentence may be unavoidable?
if it is to                         % phrase should be "to" (usually followed by "be X")
if they are to                      % phrase should be "to" (usually followed by "be X")
in general                          % phrase unless matched with "in specific," this is usually useless; perhaps "overall"
in order to                         % phrase remove "in order" and get "to"
in the past                         % phrase past tense is likely enough.
in the way of                       % phrase should be "as"
counting the number of              % phrase counting.  dude.
is permitted to                     % phrase "may"
largely opaque                      % phrase largely does not modify opaque
makes a new                         % phrase should be "creates"
may not chose                       % phrase "may not" is future tense; "chose" is past.
one should note                     % phrase just write it.
note that                           % phrase is the rest of the paper less notable?
Note, that                          % syntax not only should you not "note that", no comma after note.
we note                             % phrase is the rest of the paper less notable?
note however that                   % phrase is the rest of the paper less notable?
it is important to note             % phrase is the rest of the paper less notable?
really                              % phrase probably doesn't add; if you think it does, use "r{}eally" -- don't change to 'in fact'
in fact				    % phrase cut
rigorously                          % spelling probably doesn't add, and I rarely do anything with rigor
the way in which                    % phrase should be "how" or ""
the manner in which                 % phrase should be "how" or ""
value stems                         % phrase value is derived or offered, I think.
time at which                       % phrase very likely "when"
place at which                      % phrase very likely "where"
at the time                         % phrase very likely "when"
reduced number of                   % phrase very likely "fewer" or maybe maybe "less"
is present in                       % phrase present is probably redudant, try "is in"
they all                            % phrase maybe "all xs" would be better.
easy to do                          % phrase "feasible" or "practical" might be better.
is going to                         % phrase "will".
are going to                        % phrase "will".
getting                             % phrase probably "receiving" or "querying"
those are                           % phrase see if "those X are" is clearer?
design is motivated                 % phrase "inspired by" is probably better than "motivated" for design
locations throughout the world      % phrase drop "throughout the world"
e.g., as opposed to                 % phrase if you're giving examples, you're not talking about what isn't.  drop "e.g."
in addition, we also                % phrase remove either "also" or "in addition"
other related issues                % phrase probably remove "other"
the aforementioned                  % phrase "these xs" or "this x" would be less snooty
center around                       % phrase (cook) a center is a point: "center on" is okay.
could care less                     % phrase (cook) 'really? how much less could you care?' (should be couldn't)
grouped together                    % phrase redundant.  "grouped" alone should suffice.
put together                        % phrase long: "construct" "build" or "assemble"
consistent with each other          % phrase redundant.  "consistent" suffices.
be accomplished with                % phrase try "requires" "uses" "needs"?
the lack of knowledge of            % phrase would "X is unknown" work better?
gets to know                        % phrase you mean "learns"
trying to look like                 % phrase you mean "acting", "emulating", or "mimicing"
has got to be                       % phrase "must be"
got                                 % phrase try "became" "received" ?
gotten                              % phrase try "helped" ?
live in a vacuum                    % phrase a tired metaphor that makes me want to vomit.
positive impact                     % phrase try "benefit"
negative impact                     % phrase try "harm" or "consequences"
adverse impact                      % phrase try "harm" or "consequences"
adversely impacting                 % phrase try "harming" or "hurting"
discuss the issues of               % phrase could probably drop "the issues of" unless there's a list
the presence of                     % phrase not far from 'is', 'has', etc.
does not allow                      % phrase consider "forbids" or "prohibits"
and/or                              % phrase just say or.
there is the potential to           % phrase just say may.
there is the possibility that       % phrase just say might.
can be achieved                     % phrase maybe not so good?
find out                            % phrase perhaps determine?
in the absence of                   % phrase perhaps without?
in the presence of                  % phrase perhaps with?
set up                              % phrase perhaps create, configure, or initialize
in the face of                      % phrase can be overused.  try despite?
several times (at|of)               % phrase discouraged by Kurt.
a large degree of                   % phrase ick.
we start by first                   % phrase redundant. ("first, we" or "we start by").
in general, they are usually        % phrase redundant.
refers to the notion                % phrase define your term precisely if possible.
a significant amount of             % phrase probably just "significant"
real practical                      % phrase as opposed to imaginary practical?
people that are                     % phrase use people who are?
additional detail that we add       % phrase as opposed to additional detail that we subtract?
in some cases and not in others     % phrase "in some cases"
it is known that                    % phrase just say it.
caused due to                       % phrase "caused by"
a result of the fact that           % phrase "caused by"
results (indicate|show|suggest)     % phrase drop
research (indicates|show|suggest)   % phrase drop
can be attributed to the fact that  % phrase "is because"
a large set of                      % phrase probably don't care that it is a set.
a small set of                      % phrase probably don't care that it is a set: use 'a few'
provides a look at                  % phrase (timid) probably mean "shows".
in most cases                       % phrase "usually"
continue into the forseeable future % phrase "continue".
for the forseeable future           % phrase drop.
fail to successfully                % phrase "fail to" is sufficient.
Clearly,                            % syntax starting a sentence with clearly confuses me.
in different continents             % phrase ON different continents, IN different countries
(we|to) handle                      % phrase use a more specific verb like address, treat, solve
handling                            % phrase use a more specific verb like addressing, treating, solving, mitigating (unless handling errors or exceptions)
For the purposes of                 % phrase "For"
We observe that                     % phrase drop.
some degree of                      % phrase "some"
in the problem of                   % phrase (contributed by rap)
conclude several things             % phrase make (draw) several conclusions
extra bonus                         % phrase "bonus"
added bonus                         % phrase "bonus"
it is important to emphasize that   % phrase use diction to emphasize.
it is possible that                 % phrase "x may y"
caused due to                       % phrase "caused by"
recent work by                      % phrase could maybe be dropped, as the cite will include the date.
identify the location of            % phrase "find"
that go across                      % phrase "that cross"
ideally, we would like              % phrase "we would like"
enabling the ability to             % phrase "supporting" or "allowing" or "permitting"
absolutely essential                % phrase essential is.
we essentially do                   % phrase essentially is a poor adverb.  "The essence of our algorithm is a..."
Essentially,                        % phrase maybe "In essence," but could also be removed.
In this section (we|I)              % phrase "In this section, we", or "In this section, I"
essentially all                     % phrase "most"
past experience                     % phrase "experience" http://www.cmu.edu/styleguide/trickywords.html
particulary difficult primarily     % phrase simplify
intuition about why                 % phrase "intuition as to why"
Recall from above                   % phrase "recall"
Further, (I|we) will also           % phrase drop further or also
respectively                        % phrase unneeded.
in terms of                         % phrase don't need this.
the extent to which                 % phrase "how much"
make sure                           % phrase "ensure"
make up                             % phrase "constitute" "compose"
make use of                         % phrase "use"
make a decision                     % phrase "decide"
make a guess                        % phrase "guess"
since that time                     % phrase "since then"
choices to make                     % phrase "choices"
certain limitations                 % phrase what does 'certain' add to limitations?
will [a-z]* in the future           % phrase "will"
business entities                   % phrase "businesses"
rely primarily on                   % phrase "primarily" weakens "rely".  perhaps just "use" would be simpler.
has the potential to                % phrase can
have not yet developed              % phrase "have yet to develop"
to be effective,                    % phrase probably redundant.
provide information about           % phrase "tell how" "reveal" "expose" "disclose"
are different,                      % phrase "differ"
have already been                   % phrase "have been"? "were"?
as appropriate                      % phrase not needed?
only rarely                         % phrase "rarely" is probably enough.
is effective at                     % phrase "can"
foremost among them is              % phrase "foremost is" would be shorter.
those that have no                  % phrase those without
that have no                        % phrase "without"?
a variety of diverse                % phrase redundant
be highly valuable in               % phrase simplify.
the overall goal                    % phrase 'the goal'
sometimes an? [a-z]+ will           % phrase an x may
this is perhaps because             % phrase this may be because
adding an additional                % phrase redundant
IP protocol                         % phrase redundant
works well                          % phrase be more specific.
something                           % phrase could eliminate.
to keep from                        % phrase "to avoid"
[\.,] since (!then)                 % phrase probably you mean "because" unless you're talking about time. -- "has since" is okay.
performance characteristics         % phrase rare that characteristics adds.
takes into account                  % phrase considers
specify particular                  % phrase if specifying, particular should be redundant.
prototype implementation            % phrase "implementation" is redundant.
given a particular                  % phrase "given a" is probably enough
described in detail (in|below)      % phrase use "detailed"
relatively more                     % phrase more is already relative.
focus primarily on                  % phrase bad metaphor: subject of focus is singular.
primary focus                       % phrase bad metaphor: subject of focus is singular.
relatively more                     % phrase more is already relative.
gives [a-z]+ [a-z]+ information about % phrase use "tells" x
gives [a-z]+ information about      % phrase use "tells" x
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
have an effect on                   % phrase "affect"
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
we can see                          % phrase "we can see" isn't formal enough.
still remain                        % phrase "remain".
change over time                    % phrase "change"
turn into                           % phrase "become"
looking back in retrospect          % phrase pick.
ensures that there will be no       % phrase "prevents"
does have                           % phrase "has"
first step toward this              % phrase "toward this" can probably be dropped.
can potentially be                  % phrase "might be", or just "can be"
obviates the need for               % phrase just obviates x, not obviates the need for x.
it is indeed                        % phrase "it is", though still passive.
planning in advance                 % phrase when else might you plan?
a lot of                            % phrase "many"
keep in mind                        % phrase "consider" (or drop)
it is clear that                    % phrase if clear, you don't have to say it.
especially true                     % phrase true is an absolute, can't be especially true.
making it increasingly difficult    % phrase preventing, discouraging, impeding, blocking, slowing...
is potentially                      % phrase "may be"
have been [a-z]* in the past        % phrase 'in the past' is redundant with tense.
amount of time  % phrase "duration"
should ideally % phrase "should"
are of great benefit to % phrase "help" or "aid"
are of benefit to % phrase "help" or "aid" or "promote"
important here % phrase consider "relevant"
while at the same time % phrase "while" is enough.
are able to % phrase can
subvert the proper operation of % phrase subvert
speed slow % phrase speed is probably redundant.
of size no smaller than % phrase "of size" is probably redundant
of size no larger than % phrase "of size" is probably redundant
of size smaller than % phrase "of size" is probably redundant
of size larger than % phrase "of size" is probably redundant
might potentially % phrase "might"
in the context of % phrase "in" avoid, if possible.
increase the amount of % phrase probably just increase.
show the difference between % phrase compare
in addition, we also % phrase pick.
overhead efficiency % phrase huh?
have an effect on % phrase "affect"
have a signficant effect on %  phrase "affect"
we find % phrase can usually be removed
this suggests % phrase remove or make more precise
effective for providing	   	 % phrase remove
we performed a                   % phrase just use the verb directly
we perform a                     % phrase just use the verb directly
were able to                     % phrase could
are able to                      % phrase can


==> sections/ACL_template.tex <==

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{wanrong.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{wanrong}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,wanrong}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.
